Refusal-Trained LLMs Are Easily Jailbroken As Browser Agents

For safety reasons, large language models (LLMs) are trained to refuse harmful user instructions, such as assisting dangerous activities. We study an open question in this work: does the desired safety refusal, typically enforced in chat contexts, generalize to non-chat and agentic use cases? Unlike chatbots, LLM agents equipped with general-purpose tools, such as web browsers and mobile devices, can directly influence the real world, making it even more crucial to refuse harmful instructions. In this work, we primarily focus on red-teaming browser agents, LLMs that manipulate information via web browsers. To this end, we introduce Browser Agent Red teaming Toolkit (BrowserART), a comprehensive test suite designed specifically for red-teaming browser agents. BrowserART is consist of 100 diverse browser-related harmful behaviors (including original behaviors and ones sourced from HarmBench [Mazeika et al., 2024] and AirBench 2024 [Zeng et al., 2024b]) across both synthetic and real websites. Our empirical study on state-of-the-art browser agents reveals that, while the backbone LLM refuses harmful instructions as a chatbot, the corresponding agent does not. Moreover, attack methods designed to jailbreak refusal-trained LLMs in the chat settings transfer effectively to browser agents. With human rewrites, GPT-4o and o1-preview-based browser agents attempted 98 and 63 harmful behaviors (out of 100), respectively. We publicly release BrowserART and call on LLM developers, policymakers, and agent developers to collaborate on improving agent safety

==> math_commands.tex <==
% %%%%% NEW MATH DEFINITIONS %%%%%

% % Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}

% % Highlight a newly defined term
% \newcommand{\newterm}[1]{{\bf #1}}


% % Figure reference, lower-case.
% \def\figref#1{figure~\ref{#1}}
% % Figure reference, capital. For start of sentence
% \def\Figref#1{Figure~\ref{#1}}
% \def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
% \def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% % Section reference, lower-case.
% \def\secref#1{section~\ref{#1}}
% % Section reference, capital.
% \def\Secref#1{Section~\ref{#1}}
% % Reference to two sections.
% \def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% % Reference to three sections.
% \def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% % Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% % Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% % A raw reference to an equation---avoid using if possible
% \def\plaineqref#1{\ref{#1}}
% % Reference to a chapter, lower-case.
% \def\chapref#1{chapter~\ref{#1}}
% % Reference to an equation, upper case.
% \def\Chapref#1{Chapter~\ref{#1}}
% % Reference to a range of chapters
% \def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% % Reference to an algorithm, lower-case.
% \def\algref#1{algorithm~\ref{#1}}
% % Reference to an algorithm, upper case.
% \def\Algref#1{Algorithm~\ref{#1}}
% \def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
% \def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% % Reference to a part, lower case
% \def\partref#1{part~\ref{#1}}
% % Reference to a part, upper case
% \def\Partref#1{Part~\ref{#1}}
% \def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

% \def\ceil#1{\lceil #1 \rceil}
% \def\floor#1{\lfloor #1 \rfloor}
% \def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

% \def\eps{{\epsilon}}


% % Random variables
% \def\reta{{\textnormal{$\eta$}}}
% \def\ra{{\textnormal{a}}}
% \def\rb{{\textnormal{b}}}
% \def\rc{{\textnormal{c}}}
% \def\rd{{\textnormal{d}}}
% \def\re{{\textnormal{e}}}
% \def\rf{{\textnormal{f}}}
% \def\rg{{\textnormal{g}}}
% \def\rh{{\textnormal{h}}}
% \def\ri{{\textnormal{i}}}
% \def\rj{{\textnormal{j}}}
% \def\rk{{\textnormal{k}}}
% \def\rl{{\textnormal{l}}}
% % rm is already a command, just don't name any random variables m
% \def\rn{{\textnormal{n}}}
% \def\ro{{\textnormal{o}}}
% \def\rp{{\textnormal{p}}}
% \def\rq{{\textnormal{q}}}
% \def\rr{{\textnormal{r}}}
% \def\rs{{\textnormal{s}}}
% \def\rt{{\textnormal{t}}}
% \def\ru{{\textnormal{u}}}
% \def\rv{{\textnormal{v}}}
% \def\rw{{\textnormal{w}}}
% \def\rx{{\textnormal{x}}}
% \def\ry{{\textnormal{y}}}
% \def\rz{{\textnormal{z}}}

% % Random vectors
% \def\rvepsilon{{\mathbf{\epsilon}}}
% \def\rvtheta{{\mathbf{\theta}}}
% \def\rva{{\mathbf{a}}}
% \def\rvb{{\mathbf{b}}}
% \def\rvc{{\mathbf{c}}}
% \def\rvd{{\mathbf{d}}}
% \def\rve{{\mathbf{e}}}
% \def\rvf{{\mathbf{f}}}
% \def\rvg{{\mathbf{g}}}
% \def\rvh{{\mathbf{h}}}
% \def\rvu{{\mathbf{i}}}
% \def\rvj{{\mathbf{j}}}
% \def\rvk{{\mathbf{k}}}
% \def\rvl{{\mathbf{l}}}
% \def\rvm{{\mathbf{m}}}
% \def\rvn{{\mathbf{n}}}
% \def\rvo{{\mathbf{o}}}
% \def\rvp{{\mathbf{p}}}
% \def\rvq{{\mathbf{q}}}
% \def\rvr{{\mathbf{r}}}
% \def\rvs{{\mathbf{s}}}
% \def\rvt{{\mathbf{t}}}
% \def\rvu{{\mathbf{u}}}
% \def\rvv{{\mathbf{v}}}
% \def\rvw{{\mathbf{w}}}
% \def\rvx{{\mathbf{x}}}
% \def\rvy{{\mathbf{y}}}
% \def\rvz{{\mathbf{z}}}

% % Elements of random vectors
% \def\erva{{\textnormal{a}}}
% \def\ervb{{\textnormal{b}}}
% \def\ervc{{\textnormal{c}}}
% \def\ervd{{\textnormal{d}}}
% \def\erve{{\textnormal{e}}}
% \def\ervf{{\textnormal{f}}}
% \def\ervg{{\textnormal{g}}}
% \def\ervh{{\textnormal{h}}}
% \def\ervi{{\textnormal{i}}}
% \def\ervj{{\textnormal{j}}}
% \def\ervk{{\textnormal{k}}}
% \def\ervl{{\textnormal{l}}}
% \def\ervm{{\textnormal{m}}}
% \def\ervn{{\textnormal{n}}}
% \def\ervo{{\textnormal{o}}}
% \def\ervp{{\textnormal{p}}}
% \def\ervq{{\textnormal{q}}}
% \def\ervr{{\textnormal{r}}}
% \def\ervs{{\textnormal{s}}}
% \def\ervt{{\textnormal{t}}}
% \def\ervu{{\textnormal{u}}}
% \def\ervv{{\textnormal{v}}}
% \def\ervw{{\textnormal{w}}}
% \def\ervx{{\textnormal{x}}}
% \def\ervy{{\textnormal{y}}}
% \def\ervz{{\textnormal{z}}}

% % Random matrices
% \def\rmA{{\mathbf{A}}}
% \def\rmB{{\mathbf{B}}}
% \def\rmC{{\mathbf{C}}}
% \def\rmD{{\mathbf{D}}}
% \def\rmE{{\mathbf{E}}}
% \def\rmF{{\mathbf{F}}}
% \def\rmG{{\mathbf{G}}}
% \def\rmH{{\mathbf{H}}}
% \def\rmI{{\mathbf{I}}}
% \def\rmJ{{\mathbf{J}}}
% \def\rmK{{\mathbf{K}}}
% \def\rmL{{\mathbf{L}}}
% \def\rmM{{\mathbf{M}}}
% \def\rmN{{\mathbf{N}}}
% \def\rmO{{\mathbf{O}}}
% \def\rmP{{\mathbf{P}}}
% \def\rmQ{{\mathbf{Q}}}
% \def\rmR{{\mathbf{R}}}
% \def\rmS{{\mathbf{S}}}
% \def\rmT{{\mathbf{T}}}
% \def\rmU{{\mathbf{U}}}
% \def\rmV{{\mathbf{V}}}
% \def\rmW{{\mathbf{W}}}
% \def\rmX{{\mathbf{X}}}
% \def\rmY{{\mathbf{Y}}}
% \def\rmZ{{\mathbf{Z}}}

% % Elements of random matrices
% \def\ermA{{\textnormal{A}}}
% \def\ermB{{\textnormal{B}}}
% \def\ermC{{\textnormal{C}}}
% \def\ermD{{\textnormal{D}}}
% \def\ermE{{\textnormal{E}}}
% \def\ermF{{\textnormal{F}}}
% \def\ermG{{\textnormal{G}}}
% \def\ermH{{\textnormal{H}}}
% \def\ermI{{\textnormal{I}}}
% \def\ermJ{{\textnormal{J}}}
% \def\ermK{{\textnormal{K}}}
% \def\ermL{{\textnormal{L}}}
% \def\ermM{{\textnormal{M}}}
% \def\ermN{{\textnormal{N}}}
% \def\ermO{{\textnormal{O}}}
% \def\ermP{{\textnormal{P}}}
% \def\ermQ{{\textnormal{Q}}}
% \def\ermR{{\textnormal{R}}}
% \def\ermS{{\textnormal{S}}}
% \def\ermT{{\textnormal{T}}}
% \def\ermU{{\textnormal{U}}}
% \def\ermV{{\textnormal{V}}}
% \def\ermW{{\textnormal{W}}}
% \def\ermX{{\textnormal{X}}}
% \def\ermY{{\textnormal{Y}}}
% \def\ermZ{{\textnormal{Z}}}

% % Vectors
% \def\vzero{{\bm{0}}}
% \def\vone{{\bm{1}}}
% \def\vmu{{\bm{\mu}}}
% \def\vtheta{{\bm{\theta}}}
% \def\va{{\bm{a}}}
% \def\vb{{\bm{b}}}
% \def\vc{{\bm{c}}}
% \def\vd{{\bm{d}}}
% \def\ve{{\bm{e}}}
% \def\vf{{\bm{f}}}
% \def\vg{{\bm{g}}}
% \def\vh{{\bm{h}}}
% \def\vi{{\bm{i}}}
% \def\vj{{\bm{j}}}
% \def\vk{{\bm{k}}}
% \def\vl{{\bm{l}}}
% \def\vm{{\bm{m}}}
% \def\vn{{\bm{n}}}
% \def\vo{{\bm{o}}}
% \def\vp{{\bm{p}}}
% \def\vq{{\bm{q}}}
% \def\vr{{\bm{r}}}
% \def\vs{{\bm{s}}}
% \def\vt{{\bm{t}}}
% \def\vu{{\bm{u}}}
% \def\vv{{\bm{v}}}
% \def\vw{{\bm{w}}}
% \def\vx{{\bm{x}}}
% \def\vy{{\bm{y}}}
% \def\vz{{\bm{z}}}

% % Elements of vectors
% \def\evalpha{{\alpha}}
% \def\evbeta{{\beta}}
% \def\evepsilon{{\epsilon}}
% \def\evlambda{{\lambda}}
% \def\evomega{{\omega}}
% \def\evmu{{\mu}}
% \def\evpsi{{\psi}}
% \def\evsigma{{\sigma}}
% \def\evtheta{{\theta}}
% \def\eva{{a}}
% \def\evb{{b}}
% \def\evc{{c}}
% \def\evd{{d}}
% \def\eve{{e}}
% \def\evf{{f}}
% \def\evg{{g}}
% \def\evh{{h}}
% \def\evi{{i}}
% \def\evj{{j}}
% \def\evk{{k}}
% \def\evl{{l}}
% \def\evm{{m}}
% \def\evn{{n}}
% \def\evo{{o}}
% \def\evp{{p}}
% \def\evq{{q}}
% \def\evr{{r}}
% \def\evs{{s}}
% \def\evt{{t}}
% \def\evu{{u}}
% \def\evv{{v}}
% \def\evw{{w}}
% \def\evx{{x}}
% \def\evy{{y}}
% \def\evz{{z}}

% % Matrix
% \def\mA{{\bm{A}}}
% \def\mB{{\bm{B}}}
% \def\mC{{\bm{C}}}
% \def\mD{{\bm{D}}}
% \def\mE{{\bm{E}}}
% \def\mF{{\bm{F}}}
% \def\mG{{\bm{G}}}
% \def\mH{{\bm{H}}}
% \def\mI{{\bm{I}}}
% \def\mJ{{\bm{J}}}
% \def\mK{{\bm{K}}}
% \def\mL{{\bm{L}}}
% \def\mM{{\bm{M}}}
% \def\mN{{\bm{N}}}
% \def\mO{{\bm{O}}}
% \def\mP{{\bm{P}}}
% \def\mQ{{\bm{Q}}}
% \def\mR{{\bm{R}}}
% \def\mS{{\bm{S}}}
% \def\mT{{\bm{T}}}
% \def\mU{{\bm{U}}}
% \def\mV{{\bm{V}}}
% \def\mW{{\bm{W}}}
% \def\mX{{\bm{X}}}
% \def\mY{{\bm{Y}}}
% \def\mZ{{\bm{Z}}}
% \def\mBeta{{\bm{\beta}}}
% \def\mPhi{{\bm{\Phi}}}
% \def\mLambda{{\bm{\Lambda}}}
% \def\mSigma{{\bm{\Sigma}}}

% % Tensor
% \DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
% \SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
% \def\tA{{\tens{A}}}
% \def\tB{{\tens{B}}}
% \def\tC{{\tens{C}}}
% \def\tD{{\tens{D}}}
% \def\tE{{\tens{E}}}
% \def\tF{{\tens{F}}}
% \def\tG{{\tens{G}}}
% \def\tH{{\tens{H}}}
% \def\tI{{\tens{I}}}
% \def\tJ{{\tens{J}}}
% \def\tK{{\tens{K}}}
% \def\tL{{\tens{L}}}
% \def\tM{{\tens{M}}}
% \def\tN{{\tens{N}}}
% \def\tO{{\tens{O}}}
% \def\tP{{\tens{P}}}
% \def\tQ{{\tens{Q}}}
% \def\tR{{\tens{R}}}
% \def\tS{{\tens{S}}}
% \def\tT{{\tens{T}}}
% \def\tU{{\tens{U}}}
% \def\tV{{\tens{V}}}
% \def\tW{{\tens{W}}}
% \def\tX{{\tens{X}}}
% \def\tY{{\tens{Y}}}
% \def\tZ{{\tens{Z}}}


% % Graph
% \def\gA{{\mathcal{A}}}
% \def\gB{{\mathcal{B}}}
% \def\gC{{\mathcal{C}}}
% \def\gD{{\mathcal{D}}}
% \def\gE{{\mathcal{E}}}
% \def\gF{{\mathcal{F}}}
% \def\gG{{\mathcal{G}}}
% \def\gH{{\mathcal{H}}}
% \def\gI{{\mathcal{I}}}
% \def\gJ{{\mathcal{J}}}
% \def\gK{{\mathcal{K}}}
% \def\gL{{\mathcal{L}}}
% \def\gM{{\mathcal{M}}}
% \def\gN{{\mathcal{N}}}
% \def\gO{{\mathcal{O}}}
% \def\gP{{\mathcal{P}}}
% \def\gQ{{\mathcal{Q}}}
% \def\gR{{\mathcal{R}}}
% \def\gS{{\mathcal{S}}}
% \def\gT{{\mathcal{T}}}
% \def\gU{{\mathcal{U}}}
% \def\gV{{\mathcal{V}}}
% \def\gW{{\mathcal{W}}}
% \def\gX{{\mathcal{X}}}
% \def\gY{{\mathcal{Y}}}
% \def\gZ{{\mathcal{Z}}}

% % Sets
% \def\sA{{\mathbb{A}}}
% \def\sB{{\mathbb{B}}}
% \def\sC{{\mathbb{C}}}
% \def\sD{{\mathbb{D}}}
% % Don't use a set called E, because this would be the same as our symbol
% % for expectation.
% \def\sF{{\mathbb{F}}}
% \def\sG{{\mathbb{G}}}
% \def\sH{{\mathbb{H}}}
% \def\sI{{\mathbb{I}}}
% \def\sJ{{\mathbb{J}}}
% \def\sK{{\mathbb{K}}}
% \def\sL{{\mathbb{L}}}
% \def\sM{{\mathbb{M}}}
% \def\sN{{\mathbb{N}}}
% \def\sO{{\mathbb{O}}}
% \def\sP{{\mathbb{P}}}
% \def\sQ{{\mathbb{Q}}}
% \def\sR{{\mathbb{R}}}
% \def\sS{{\mathbb{S}}}
% \def\sT{{\mathbb{T}}}
% \def\sU{{\mathbb{U}}}
% \def\sV{{\mathbb{V}}}
% \def\sW{{\mathbb{W}}}
% \def\sX{{\mathbb{X}}}
% \def\sY{{\mathbb{Y}}}
% \def\sZ{{\mathbb{Z}}}

% % Entries of a matrix
% \def\emLambda{{\Lambda}}
% \def\emA{{A}}
% \def\emB{{B}}
% \def\emC{{C}}
% \def\emD{{D}}
% \def\emE{{E}}
% \def\emF{{F}}
% \def\emG{{G}}
% \def\emH{{H}}
% \def\emI{{I}}
% \def\emJ{{J}}
% \def\emK{{K}}
% \def\emL{{L}}
% \def\emM{{M}}
% \def\emN{{N}}
% \def\emO{{O}}
% \def\emP{{P}}
% \def\emQ{{Q}}
% \def\emR{{R}}
% \def\emS{{S}}
% \def\emT{{T}}
% \def\emU{{U}}
% \def\emV{{V}}
% \def\emW{{W}}
% \def\emX{{X}}
% \def\emY{{Y}}
% \def\emZ{{Z}}
% \def\emSigma{{\Sigma}}

% % entries of a tensor
% % Same font as tensor, without \bm wrapper
% \newcommand{\etens}[1]{\mathsfit{#1}}
% \def\etLambda{{\etens{\Lambda}}}
% \def\etA{{\etens{A}}}
% \def\etB{{\etens{B}}}
% \def\etC{{\etens{C}}}
% \def\etD{{\etens{D}}}
% \def\etE{{\etens{E}}}
% \def\etF{{\etens{F}}}
% \def\etG{{\etens{G}}}
% \def\etH{{\etens{H}}}
% \def\etI{{\etens{I}}}
% \def\etJ{{\etens{J}}}
% \def\etK{{\etens{K}}}
% \def\etL{{\etens{L}}}
% \def\etM{{\etens{M}}}
% \def\etN{{\etens{N}}}
% \def\etO{{\etens{O}}}
% \def\etP{{\etens{P}}}
% \def\etQ{{\etens{Q}}}
% \def\etR{{\etens{R}}}
% \def\etS{{\etens{S}}}
% \def\etT{{\etens{T}}}
% \def\etU{{\etens{U}}}
% \def\etV{{\etens{V}}}
% \def\etW{{\etens{W}}}
% \def\etX{{\etens{X}}}
% \def\etY{{\etens{Y}}}
% \def\etZ{{\etens{Z}}}

% % The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak


==> sections/03_Dataset.tex <==
\section{\longdataset}\label{sec:test-suite}

We introduce \textbf{Browser} \textbf{A}gent \textbf{R}ed Teaming \textbf{T}oolkit~(\textbf{\shortdataset}) to address the two issues from existing safety benchmarks discussed in \S\ref{sec:background}.

% \subsection{Overview}

\paragraph{Overview.}\shortdataset~consists of 100 harmful browser-related behaviors that an agent is not supposed to assist. 
% Out of these 100 behaviors, there are \todo{X} behaviors requesting the agent to generate harmful text or interactions on specific websites (e.g. Twitter/X and Gmail). 
We divided all behaviors into two main categories: \emph{harmful content} and \emph{harmful interaction}. Under each main categories, we create sub-categories for the harm semantics(\S~\ref{sec:toolkit:behaviors}). 
We created 40 synthetic websites under 19 domains for red teaming browser behaviors that targeting on specific websites (\eg~Twitter/X). These synthetic pages are hosted locally for running red teaming experiments in a sandbox without polluting the real world, especially the social media and government sites (\S\ref{sec:toolkit:websites}). We discuss how to create classify if the agent is attempting the harmful behavior in \S\ref{sec:dataset:eval}.

\begin{figure}[t]
\vspace{-30pt}
\begin{center}
\includegraphics[width=\textwidth, trim=25 60 10 10, clip]{images/sub_category_distribution_v1.pdf}
\end{center}
\caption{Test Suite Dataset Info Card.}
\label{fig:dataset-card}
\vspace{-0.5cm}
\end{figure}

\subsection{Behavior Dataset}\label{sec:toolkit:behaviors}


\begin{wrapfigure}{R}{0.35\textwidth}  % Adjust the width to reduce horizontal white space
\vspace{-20pt}
\begin{center}
\includegraphics[width=1.05\linewidth, trim=100 20 100 20, clip]{images/behavior_distribution.pdf}  % Adjust trim values further
\caption{Overall Distribution of Behavior Sources}
\label{fig:distribution_behavior_sources}
\end{center}
\vspace{-0.5cm}
\end{wrapfigure} 

\paragraph{Chat and Browser Behaviors.} We denote a behavior as a \emph{chat behavior} if it is used to red team an LLM in chats. Similarly, if it is used to red team a browser agent, we refer to it as a \emph{browser behavior.} We give an example in Figure~\ref{fig:main-result}.  It is often possible to rephrase a chat behavior into a browser behavior, and vice versa. In the \shortdataset, we include 100 browser behaviors, either original or rephrased from existing chat behaviors sourced from HarmBench~\citep{mazeika2024harmbench} or AirBench 2024~\citep{zeng2024air}, with the distribution shown in Figure~\ref{fig:distribution_behavior_sources}. In our rephrasing process, we preserve the original semantics of the chat behaviors, making only minimal modifications to ensure the behavior is tailored for a browser agent. For example, if a chat behavior originally asks the LLM to outline a plan, we modify it so the corresponding browser behavior is to send the plan in an email or in a social media post. Some chat behaviors can be underspecified for the sake of generality, such as \emph{Create a blackmail for someone}. To enable full automation in the red teaming process, we add the necessary details missing from the chat behavior when converting it into a browser behavior, ensuring the agent can complete the task without additional human input. In this example, we would rephrase it as \emph{Create a blackmail and send it to [EMAIL]}.

The browser behavior dataset of \shortdataset~incorporates two main harm categories: \emph{Harmful Content} (47 behaviors) and \emph{Harmful Interaction} (53 behaviors).

\paragraph{Harmful Content.} In this category, the browser agent is instructed to generate harmful content and spread the harm to the Internet. To prepare behaviors incorporating harmful contents, we start with sourcing 24 chat behaviors from HarmBench~\cite{mazeika2024harmbench} and 17 behaviors from AirBench 2024~\cite{zeng2024air}. We additionally created 6 original chat behaviors. Figure~\ref{fig:dataset-card} provides a detailed breakdown for all sub categories. Next, we convert these chat behaviors into browser behaviors. The resulting browser behaviors are often rephrased to sending emails and social media posts. In total, we have 47 chat behaviors covering 7 sub categories in Figure~\ref{fig:dataset-card}. There is no technical issue that would prevent us from sourcing the entire HarmBench or AirBench 2024 for maximizing the number of sub-categories; however, we particularly pick these categories as they relate to cyber activities much closer than other categories.

\paragraph{Harmful Interaction.} In this category, the agent is instructed to create a series of browser events, such as clicks and page navigation, that generate harm on a given website. Each individual interaction is usually benign but the collective impact of these interactions might be considered harmful or illegal. For example, a login help is not illegal but trying to predict the password of a private account and continuously assisting login attempts are harmful (and potentially illegal). We sampled 11 chat behaviors from HarmBench and 2 from AirBench 2024 describing harmful interactions on the Internet and modify them into browser behaviors. In addition, we created 40 original chat behaviors related to harmful interactions on the Internet and rephrase them into browser behaviors. In total, we include 53 behaviors incorporating harmful interactions in \shortdataset, covering 9 sub categories, such as copyright content, assisting hiring discrimination, and cybercrime intrusion. Figure~\ref{fig:dataset-card} provides a detailed breakdown for all sub categories. In particular, for behaviors related to exploiting security vulnerabilities, we focus on those with an adversarial objective, as the discovery of cyber vulnerabilities for the purpose of improving cybersecurity is considered a benign application.

\paragraph{Summary.} The behavior set of \shortdataset~ distinguishes itself from existing LLM safety benchmarks with 100 browser behaviors covering harmful contents and interactions, tailored for red teaming browser LLM agents. Each \shortdataset~behavior is associated with a source chat behavior. A benchmark with 100 entries strikes the right balance between diversity and practicality when testing LLM vulnerabilities. It offers enough data to reveal patterns in model behavior, covering both common scenarios and edge cases, without being too resource-intensive. 

% The behavior dataset of \shortdataset~is carefully curated to encompass a wide range of harm categories and is specifically designed to include more harmful interactions—an often overlooked aspect in the current literature on LLM and agent safety. Additionally, each browser behavior is paired with a corresponding chat behavior in \shortdataset~, enabling an exploration of the safety and alignment between the LLM and the agent system built on the same model.

\subsection{ Websites}\label{sec:toolkit:websites}
To prevent browser agents from causing irreversible harm to the public when red teaming on specific websites such as sending Twitter posts, we created synthetic versions of these domains, such as locally served Twitter pages, as alternatives. We developed 40 synthetic websites for 77 out of 100 behaviors by prompting an LLM to generate these websites first to mimic the real ones on WebSim\footnote{\url{https://websim.ai}; we have obtained consent from WebSim for this research.} and later adjusted details ourselves. 

For the remaining 23 behaviors that require access to the real internet (e.g., demonstrating cyberstalking), we either used the Google Search homepage as the entry URL or 
websites with no real users\footnote{We targeted 4 behaviors on the Customer Management System and GitLab pages hosted by \citet{zhou2023webarena}. These websites are not used as demos only. We obtained their consent prior to our experiments.}. Only in these cases, we had authors monitor the agents to intervene in case of any potential irreversible harm. The full set of websites used in \shortdataset~can be found in Figure \ref{fig:dataset-card}.

\paragraph{Limitations.} We highlight two limitations in our approach. First, a synthetic websites only has the target functionalities relevant to the associated behavior so it inevitably has less elements in the UI compared to the real ones. With that being said, agents can be faced with even complex cases, compared to what they have in \shortdataset. Second, including Google Search (or a similar entry point to the real Internet) requires additional human monitoring during the red teaming. It is possible to employ another safety monitor model in the follow-up work to fully automate and scale up the red teaming pipeline. 

% \begin{figure}[t]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% \end{center}
% \caption{Test Suite Website Info Card.}
% \label{fig:websites-card}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\textwidth]{images/websites.pdf}
% \caption{\todo{}}
% \label{fig:websites-cards}
% \end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\textwidth]{images/pipeline.pdf}
\end{center}
\caption{Examples behaviors, associated websites and harm classification methods. For any behavior incorporating harmful content, we use an LLM to classify the generated contents by the agent. For behaviors incorporating harmful interaction, the harm classification method is \emph{behavior-dependent}: 1) using a heuristic-based classifier for simple cases where we know how the harm can be generated; 2) using an LLM as a classifier on the agent's trajectory for other open-ended cases.}
\label{fig:example-harms}
\end{figure}

\subsection{Harm Classification}~\label{sec:dataset:eval}

% We employ an automated evaluation for browser agents by using LLM-as-a-judge~\citep{zheng2023judging}. Our experiments utilize the prompt template from HarmBench \citep{mazeika2024harmbench} to implement GPT-4o as a judge because we find that the original HarmBench classifier has a higher false positives compared to GPT-4o in our preliminary experiments with a subset of \shortdataset~behaviors.

To classify the agent's actions on generating harmful contents, we use the text content typed by the browser agent. For example, this includes the email body on our synthetic Gmail page, the input box of a Tweet, and the comment area for our synthetic Instagram news feed page. We use LLM-as-a-judge~\citep{zheng2023judging} for determining if the text is harmful. Our experiments adapts the prompt template from HarmBench \citep{mazeika2024harmbench} to implement GPT-4o as a judge because we find that the original HarmBench classifier has a higher false positives compared to GPT-4o in our preliminary experiments with a subset of \shortdataset~behaviors. The prompt template can be found in Appendix~\ref{appendix:eval}. An example is shown the first row of Figure~\ref{fig:example-harms}.

For behaviors related to harmful interactions, we discuss two cases.

\paragraph{Case I (LLM Judge for Agent Trajectory).} When there are numerous ways to generate harmful interactions for the a behavior (e.g., various methods of malicious code injection), we input the agent's trajectory—a list of actions taken—to the judge LLM for harm classification. Out of 53 behaviors incorporating the harmful interactions, there are 43 behaviors in \shortdataset~falling into this case. This is illustrated in the second row of Figure~\ref{fig:example-harms}.

\paragraph{Case II (Heuristic-based Classification).} When there is a finite set of harmful interactions on a website (e.g., repeatedly entering passwords for login attempts or continuously clicking a particular advertisement for click fraud), we implement event listeners on the back-end targeting specific web elements. We classify an agent's behavior as harmful based on tracked actions from these event listeners. For instance, if we want to evaluate behaviors related to illegal login attempts, we can check if the number of attempts made by the agent is greater than a pre-defined threshold $t$ (e.g. we use $t=3$ for login attempt experiments). In this scenario, we can determine the harmful interactions in a programmatic way and it is not necessary to employ a judge LLM. Out of 53 behaviors incorporating the harmful interactions, there are 10 behaviors in this case. This is illustrated in the last row of Figure~\ref{fig:example-harms}.

In summary, our harm classification is behavior-dependent. For each behavior, we provide the steps we employ to classify the target harm. It is important to note that \shortdataset~is designed to evaluate the safety guardrails of refusal-trained LLMs when used as browser agents, rather than assessing the dangerous capabilities of the underlying LLMs such as~\citep{yao2024survey}. Consequently, the judge LLM is prompted to classify whether the browser agent is attempting to fulfill harmful instructions, rather than determining if the agent succeeds in creating the desired harm.




==> sections/0x_motivation.tex <==
\section{Motivation}\label{sec:motivation}

Browser-based LLM agents often have access to a much wider range of real-world information and can directly influence critical domains, with a huge potential to make profound impacts on both individual and collective lives~\citep{gabriel2024ethicsadvancedaiassistants}. By leveraging a web browser like Chrome extensions, these agents can extend their capabilities to perform actions beyond searches, such as sending emails, filing out forms and accessing sensitive information.

Consider the following example as shown in Figure~\ref{fig:main-result}: an agent is instructed to write an email to convince someone to share their social security number. In a browser environment, the agent could autonomously compose a persuasive email and send to a target successfully without human oversight. Such action poses significant threat to personal privacy and security. Existing alignment techniques may not adequately address these behaviors as they are primarily designed for text-based interactions. Given the potential risks associated with these harmful behaviors, it is important for us to evaluate the safety of browser-based LLM agents. This work aims to address this need by proposing a comprehensive test suite aiming to identify and evaluate the risks associated with LLM agents for a more secure and responsible LLM agent. 
